Lagrangian Cobordism I

This paper discusses the cobordism of Lagrangian submanifolds (in the monotone setting) and structures it as a category that is related in a functorial way to an appropriate (derived) Fukaya category. Are also discussed obstructions to cobordism based on properties of Lagrangian quantum homology, relations to Lagrangian surgery, as well as examples of non-isotopic but cobordant Lagrangians. This is a revision of our earlier preprint from September 2011.

==> cat-cob.tex <==

\subsection{The category $\mathcal{C}ob^{d}(M)$}
\label{subsec:category-cob}
The purpose of this subsection is to set up Lagrangian cobordism as a
category.

We first introduce an auxiliary category
$\widetilde{{\mathcal{C}ob}^d}(M)$, $d \in K$. Its objects are
families $(L_{1}, L_{2},\ldots, L_{r})$ with $r \geq 1$, $L_{i}\in
\mathcal{L}_{d}(M)$. (Recall that $\mathcal{L}_d(M)$ stands for
the class of uniformly monotone Lagrangians $L$ with $d_L = d$, and
when $d \neq 0$ with the same monotonicity constant $\rho$ which is
omitted from the notation.)

To describe the morphisms in this category we proceed in two steps.
First, for any two horizontal isotopy classes of cobordisms $[V]$ and
$[U]$ with $V:(L'_{j}) \cobto (L_{i})$ (as in
Definition~\ref{def:Lcobordism}) and $U:(K'_{s})\cobto (K_{r})$ we
define the sum $[V]+[U]$ to be the isotopy class of a cobordism family
$W:(L'_{j})+(K'_{s})\cobto (L_{i})+(K_{r})$ so that $W=V \coprod
\widetilde{U}$ with $\widetilde{U}:(K'_{s})\cobto (K_{r})$ a cobordism
horizontally isotopic to $U$ and so that $\widetilde{U}$ is disjoint
from $V$ (to insure embeddedness we can not simply take $V$ and $U$ in
the disjoint union.) Notice that the sum $[V]+[U]$ is not commutative.

The morphisms in $\widetilde{{\mathcal{C}ob}^d}(M)$ are now defined as
follows. A morphism $$[V] \in \mor \bigl( (L'_{j})_{1 \leq j \leq S},
(L_{i})_{1\leq i\leq T} \bigr)$$ is a horizontal isotopy class that
can be written as a sum $[V]=[V_{1}] + \cdots + [V_{S}]$ with each
$V_{j}\in \mathcal{L}_{d}(\C\times M)$ a cobordism from the Lagrangian
family formed by the {\em single} Lagrangian $L'_{j}$ and a subfamily
$(L_{r(j)}, \ldots, L_{r(j)+s(j)})$ of the $(L_{i})$'s, and do that
$r(j)+s(j)+1=r(j+1)$.  In other words, $V$ decomposes as a union of
$V_{i}$'s each with a single positive end but with possibly many
negative ones. We will often denote such a morphism by $V:
(L'_{j})\longrightarrow (L_{i})$.

The composition of morphisms is induced by concatenation followed by a
rescaling to reduce the ``length'' of the cobordism to the interval
$[0,1]$. It is an easy exercise to see that this is well defined
precisely because our morphisms are (horizontal) isotopy classes of
cobordisms and because morphisms are represented by sums of cobordisms
with a single positive end.


We will consider here the void set as a Lagrangian of arbitrary
dimension. With the above conventions one would expect that the sum
operation described above gives the category
$\widetilde{{\mathcal{C}ob}^d}(M)$ the structure of a strict monoidal
category with neutral element $\emptyset$.  However, it is easy to see
that $L+\emptyset \not=\emptyset+ L$ simply because the two families
$(L,\emptyset)$ and $(\emptyset, L)$ are different. We now intend to
factor both the objects and the morphisms in this category by
equivalence relations that will transform this category in a strict
monoidal one. For the objects the equivalence relation is induced by
the relations
\begin{equation}
(L, \emptyset) \sim (\emptyset,L) \sim (L).
\label{eq:eq-objects}
\end{equation}  
 
At the level of the morphisms a bit more care is needed. For each $L
\in \mathcal{L}_{d}(M)$ we will define two particular cobordisms
$\Phi_{L}:(\emptyset, L)\cobto (L,\emptyset)$ and $\Psi_{L}:
(L,\emptyset)\cobto (\emptyset,L)$ as follows. Let $\gamma: [0,1] \to
[0,1]$ be an increasing, surjective smooth function, strictly
increasing on $(\epsilon,1-\epsilon)$ and with $\gamma'(t)=0$ for
$t\in [0,\epsilon]\cup [1-\epsilon, 1]$. We now let
$\Phi(L)=graph(\gamma)\times L$ and $\Psi(L)=graph(1-\gamma)\times L$.
The equivalence relation for morphisms is now induced by the following
two identifications:
\begin{enumerate}[(Eq 1)]
  \item For every cobordism $V$ we identify $V+\emptyset \sim
   \emptyset+V \sim V$, where $\emptyset$ is the void cobordism
   between two void Lagrangians. \label{i:eq-1}
  \item If $V:L \longrightarrow (L_{1},..., L_{i}, \emptyset,
   L_{i+2},\ldots, L_{k})$, then we identify $V \sim V' \sim V''$,
   where $V'=\Phi_{L_{i+2}} \circ V$, $V''=\Psi_{L_{i}}\circ V.$
   \label{i:eq-2}
\end{enumerate}

\begin{figure}[htbp]
   \begin{center}
      \epsfig{file=MorphCob.eps, width=0.5\linewidth}
   \end{center}
   \caption{A morphism $V:(L'_{1},L'_{2},L'_{3}) \longrightarrow
     (L_{1}, \ldots, L_{6})$, $V=V_{1}+V_{2}+V_{3}$, projected to
     $\mathbb{R}^2$.}
\end{figure}

We now construct the category $\mathcal{C}ob^{d}(M)$.  First we
consider the full subcategory $\mathcal{S}\subset
\widetilde{\cob}^{d}(M)$ obtained by restricting the objects only to
those families $(L_{1}, \ldots, L_{k})$ with $L_{i}$ non-narrow for
all $1\leq i\leq k$ (this is preferable because our functors
ultimately make use of Floer homology and we need the quantum homology
of each $L_{i}$ to be non trivial).  Then $\mathcal{C}ob^{d}(M)$ is
obtained by the quotient of the objects of $\mathcal{S}$ by the
equivalence relation in~\eqref{eq:eq-objects} and the quotient of the
morphisms of $\mathcal{S}$ by the equivalence relation
in~(Eq~\ref{i:eq-1}), (Eq~\ref{i:eq-2}).

This category is called the {\em Lagrangian cobordism category} of
$M$.  As mentioned before, it is a strict monoidal category. To
recapitulate, its objects are ordered families of non-narrow
Lagrangians $\in \mathcal{L}_{d}(M)$ and its morphisms:
$$[V]: (L'_{j}) \longrightarrow (L_{i})$$
can be represented by cobordisms $V\in\mathcal{L}_{d}(\C\times M)$ 
so that all $L_{i}$'s are
non-void and all $L'_{j}$'s are non-void except if there is just a
single $L'_{j}$ which can be void or there is just a single $L_{i}$
which can be void.  Moreover, $V$ can be written as a disjoint union
of cobordisms each with a single positive end.
 
There is a subcategory of $\mathcal{C}ob^{d}(M)$, that will be denoted
by $\mathcal{C}ob^{d}_{0}(M)$, whose objects belong to
$\mathcal{L}^{\ast}_{d}(M)$ (see~\S\ref{sb:fukaya-categ}) and whose
morphisms are represented by Lagrangian cobordisms $V$ verifying the
analogous condition to~\eqref{eq:Hlgy-vanishes}, but in $\mathbb{R}^2
\times M$. This is again a strict monoidal category.
 
% LocalWords:  embeddedness monoidal

